Terrain-Attentive Learning for Efficient 6-DoF Kinodynamic Modeling on Vertically Challenging Terrain

Wheeled robots have recently demonstrated superior mechanical capability to traverse vertically challenging terrain (e.g., extremely rugged boulders comparable in size to the vehicles themselves). Negotiating such terrain introduces significant variations of vehicle pose in all six Degrees-of-Freedom (DoFs), leading to imbalanced contact forces, varying momentum, and chassis deformation due to non-rigid tires and suspensions. To autonomously navigate on vertically challenging terrain, all these factors need to be efficiently reasoned within limited onboard computation and strict real-time constraints. In this paper, we propose a 6-DoF kinodynamics learning approach that is attentive only to the specific underlying terrain critical to the current vehicle-terrain interaction, so that it can be efficiently queried in real-time motion planners onboard small robots. Physical experiment results show our Terrain-Attentive Learning demonstrates on average 51.1% reduction in model prediction error among all 6 DoFs compared to a state-of-the-art model for vertically challenging terrain.

==> content/implementations.tex <==
\section{Implementations}
We implement \textsc{tal} on an open-source Verti-4-Wheeler (V4W) platform~\cite{datar2023toward}.
The robot is equipped with Microsoft Azure Kinect RGB-D camera, and NVIDIA Jetson Xavier, along with low-gear lockable front and rear differentials enhancing its mobility on a vertically challenging terrain.
To simulate such terrain, we used a 3.1m$\times$1.3m rock testbed with a maximum height of 0.6m.
This rock test bed facilitated the restructuring of the terrain periodically during experiments and data collection.
Specifically, we collected 30 minutes of data on the rock testbed and an additional 30 minutes of data on a planar surface. The data consists of Visual Inertia Odometry, an elevation map derived from the RGB-D input, and vehicle control data.

\subsection{Model Architecture}
To make the training easier we divided the training into three stages.
 

\textbf{Terrain attentive representation:} consists of Map encoder and Terrain Attentive Encoder.
The Map encoder is a 3-layer Convolutional Neural Network (CNN)
\label{sec::implementations}
